Build generally reusable agent-environment interaction models

This paper tackles the problem of how to pre-train a model and make it generally reusable backbones for downstream task learning. In pre-training, we propose a method that builds an agent-environment interaction model by learning domain invariant successor features from the agent's vast experiences covering various tasks, then discretize them into behavior prototypes which result in an embodied set structure. To make the model generally reusable for downstream task learning, we propose (1) embodied feature projection that retains previous knowledge by projecting the new task's observation-action pair to the embodied set structure and (2) projected Bellman updates which add learning plasticity for the new task setting. We provide preliminary results that show downstream task learning based on a pre-trained embodied set structure can handle unseen changes in task objectives, environmental dynamics and sensor modalities.

==> sections/6_model_analysis.tex <==


Next, we want to examine which part of our designed model contributes the superior performance as analyzed above. 
(1) Why SF not others, just raw state? Or VAE

(2) why use set, not directly SFs?
Number of set elements, 1 --> 50 --> 6000 --> infinity (just SFs)
The performance actually goes up and down. So set structure is better!


==> sections/method_backup.tex <==
% \subsection{Background: reusable agent-environment interaction models}
\subsection{Background: on reusable agent-environment interaction models}
%(1) 这样的model 究竟存不存在? short answers, 从传统RL的perspective，是存在，但需要大量的数据构建超大的模型，例如Bayesian world model的perspective。但是，practically，不存在。原因是MDP是这样的，要构建这个world model，不论是学representation that fits S，或是model that fits T, S, A, r, 或是policy，value， that fits, S, A, T, R, 其space的combinatorial space是大得吓人的。在这个大的world model上再做bayesian 推理，基本不可能。
% 有没有其他角度思考这个问题？这就涉及到我们的embedded agency讨论
% this paper considers a POMDP setting. 
% embedded agency怎么做到generally reusable model？ 重要的不是大，而是灵活多变。
We assume a Partial Markov Decision Process (POMDP) formation in our discussions since this setting fits in most real-world reinforcement learning tasks where the full state is not obtainable and the agent is only given observations from its onboard sensors. A POMDP is defined as a tuple $\mathcal{M}=<\mathcal{S}, \mathcal{A}, \mathcal{O}, \mathcal{T}, r, \gamma>$, where $\mathcal{S}$ is the full state space which is typically not given, $\mathcal{A}$ is the action space, $\mathcal{O}$ denotes the observation space, $\mathcal{T}$ is the transition dynamics, $r$ is the reward function that defines a task objective, $\gamma$ denotes the discount factor.


% \begin{wrapfigure}{r}{0.2\textwidth}
%     \centering
%     \includegraphics[width=0.2\textwidth]{figs/609px-Plato's_allegory_of_the_cave.jpg}\\
%     {\footnotesize Plato's allegory of the cave~\cite{Plato}. \normalsize}
%     %\label{fig:decentcem-a-architecture}
%     \vspace{-3mm}
% \end{wrapfigure}

\paragraph{Embedded agency: big world, small agent}
In 1969, Herbert Simon brought us the ``Simon's ant'' parable in chapter three of his book ``{The Science of the Artificial}''~\cite{simon1969science} that explains the complex behaviour we observed from an agent may not attribute to how complex the agent itself is, instead it results from the interaction between the agent and the complex world, while the agent like an ant, can be quite simple. This reminds us of a common setting: big world, small agent.

Unlike the \textit{Bayesian world model} approach that aims to construct a big model for the agent as a base knowledge about the big world, the \textit{Embedded agency} approach takes the perspective on how the small agent perceives, controls and gradually grows based on its own experience. Unlike a \textit{Bayesian world model} where states and models are objective, an \textit{embedded agency} approach is subjective and the agent's own bias induced from its prior experience will affect its decision-making process in both levels of state abstraction and time abstraction. This idea of intelligence closely relates to Descarte's representationalism and mind-body dualism, and to the theory of embodied embedded cognition in the philosophy of mind research. The \textit{embedded agency} approach is appealing in that it promises a scalable learning architecture to build a world model, however, it is also ambitious toward artificial general intelligence (AGI). 

This paper investigates the core idea of \textit{embedded agency} that how an agent's past experience can be used as an inductive bias to accelerate downstream task learning. We focus on a more practical starting point: in a pre-training, how to extract a model from the agent's experience that can be generally reused, as an inductive bias, to accelerate downstream task learning.  



% 从小到大进行构建。agent在环境中的behavior，受agent之前的经验所影响。（1）agent 的sensori-motor的decision建立在之前的经验上的。（2）同时，agent的handle 不同task与environment的能力是基于之前的经验可以grow的。
% embedded agency是冲着AGI去的，我们不追求这个。
% 我们关心的是一个更加practically的setting。概念上讲，embedded agency这套思路能够做到一个agent在不同环境，任务中进行学习，利用已有的experience来grow its knowledge。什么是其最simple的一个学习architecture？当我们不考虑intrinsic reward, sub-tasks, shareable skills / options, 即如何从past experience中构建知识，以及如何利用知识在下游任务中？
% embedded agency 的一个核心的思想就是agent能够construct knowledge，从experience中学习。这意味着。。。。。
% 能否将同一个agent，从不同环境，不同任务中分离出来？ 答案是不能。能分离的不是agent，而是agent与环境interaction的基础模型。
%最难以理解的就是这个agent-environment boundary。

% 一个目标，说清楚什么是从experience中学习。
% 相关， (1) agent 过去的experience 塑造了agent后续的行为决策。 

% \paragraph{Embodied agent-state construction}
% How an agent's past experience will affect its learning of a task can be generally expressed as an agent-state construction approach, where we aim to learn a function $u_{\theta}$, so that $s_{t}=u_{\theta}(x_{t}|E_{past}), \text{subject to } \mathcal{L}_{u_{\theta}}$. Here, the agent-state $s_{t}$ is a function of both current observation $x_{t}$ and the agent's past experience $E_{past}$, and $\mathcal{L}_{u_{\theta}}$ is the loss function used to optimized $u_{\theta}$ and is often hard to specify. Afterwards, $u_{\theta}$ is used in the state value function $Q^{\pi}(u_{\theta}(x_{t}), a_{t})$ task learning.

% For example, in single-task learning under the POMDP setting, we commonly use a history of previous n observation-action pairs to tackle partial observability by assuming the approximated state satisfies a Markovian property. This approach can be expressed as agent-state construction that, $s_{t}=u_{\theta}(x_{t}|\{(x_{t-k}, a_{t-k})\}_{k=1}^{n})$. Here, $E_{past}=\{(x_{t-k}, a_{t-k})\}_{k=1}^{n}$, $\mathcal{L}_{u_{\theta}}$ is the loss term measuring Markovian state property, $u_{\theta}$ is parameterized using a RNN or LSTM neural network to encode the historical data.

% In our setting, we aim to use the agent's past experience in various tasks/environments to accelerate general downstream task learning, where $s_{t}=u_{\theta}(x_{t}|\{(x_{t-k}, a_{t-k})\}_{k=1}^{n})$



% 传统agent state construction，对每一个specific task，学习u, 来 construct一个agent state。
% 我们，对所有env， task，学习，从过去的所有experience中学习如何construct agent state。
% 不再construct agent state，而是寻求construct embodied agent state，并用来支撑学习任意task，Q
% 给出我们的approach.

\paragraph{On agent-environment boundary}
% 接下来，我们解释如何学习 embodied agent-state，以及如何用它来支撑学习任意task Q.
% key insight 是，重要的不是构建一个大而通用的model，而是构建一个灵活可变的model。
% complex world, simple agent，直接提simon's ant..
% how to extract the agent out. 就是不寻求抽取agent，而是寻求抽取agent environment interaction model
% specifically, 就是抽取什么?
% 1）我们并不指望这个能够在未来agent可能遇到的所有环境，所有task都能通用。
% 2) 我们指望这个model可以继续被update，但不在这篇paper里涵盖
% 3) 这篇paper只是迈出了第一步，如何抽取一个尽量泛化的模型，以及如何应用与当初抽取用的MDP完全不同的MDP里学习。
% 4) 将来，是可以考虑更新这个embodied set模型的。
% 提出如何提取agent-environment interaction model，so that (1) M is shared across the domains. (2) M best exhibits the agent-environment interaction behaviour.
% 提出什么是generally reusable agent-environment interaction model?
% 考虑任意task，则定义一个reward-free POMDP M....，每一个generate dataset。
% 我们的目标是学习一个model = <H, T>，从数据中学习，H, T are transferrable across domains.
% 单独学习H, T很困难，若 H, T 都是transferrable，则由H, T induced的，uniform policy的successor feature也是transferrable。能否通过学习一个relaxed 版本successor feature 来得到这个generally reusable的agent-env interaction model?
% 这带来一个新的问题，如何利用sf，到downstream task学习？
% 我们知道sf本身就是有局限性的啊。这里我们用一个discretize到prototype的方法，采用feature projection, projected Bellman update 来解决这个问题。


% \paragraph{Embodied agent-state construction}
% 重要的不是构建一个大而通用的model，而是构建一个灵活可变的model。
% 对每一个specific task，学习u, 来 construct一个agent state。
% 我们，对所有env， task，学习
% The first barrier are the entangled concepts,  do not precisely align with each other

% due to the largely entangled concepts, for example,  ``embodiment'', ``embeddedness'', ``enacted'', and ``affordance'' which originated from multiple disciplines, including the philosophy of minds in cognitive science, ecological psychology in behavior science, and machine learning. To alleviate the entangled concepts barrier, this paper follows the quest proposed by~\cite{kirkpatrick2017overcoming} that we reduce the above concepts to align with a basic reinforcement leaning setting~\cite{kirkpatrick2017overcoming} 

% % except for a pool of entangled terms (for example, 
% % originated from multiple disciplines, including the philosophy of minds in cognitive science, ecological psychology in behavior science, and machine learning. 

% % that , ``embodiment'', ``embeddedness'', ``enacted'', and ``affordance'', which escalate the difficulty with extra barriers, since this research question exists in multiple disciplines, including the philosophy of minds in cognitive science, ecological psychology in behavior science, and machine learning. 

% % originated from multiple disciplines, including the philosophy of minds in cognitive science, ecological psychology in behavior science, and machine learning. 

% % that , ``embodiment'', ``embeddedness'', ``enacted'', and ``affordance'', which escalate the difficulty with extra barriers, since this research question exists in multiple disciplines, including the philosophy of minds in cognitive science, ecological psychology in behavior science, and machine learning. 

% % Following ``The quest for a common model'' proposal by Sutton et al. 2022, this paper will maintains the minimum ...  

% \paragraph{On agent-environment boundary}
% This problem is hard, this boundary is not definite, is always changing. Instead of extracting this boundary, how about extract an invariant model that is shared across all task MDPs?

% \paragraph{Embodied cognition theory}
% Explain the theory. Why this is the key to build incrementally self-improvement agent?

% \paragraph{Agent state construction}

\subsection{Pre-training: embodied agent-state construction}
% 或许这些研究最大的障碍就是过于多的名词，解释，来自己不同的领域，互相重叠又互相contradict。
We describe how to build a fundamental agent-environment interaction model using agent-state construction. The final goal is to build an embodied agent-state set, which servers as the reusable agent-environment interaction model. This set has several properties, so call it agent-environment interaction model.
There are three steps during pre-training.
\paragraph{(1) Domain labelling: Offline dataset collection modeling}

\paragraph{(2) Learn predictive representations: Extract domain invariant successor features}

\paragraph{(3) Discretize to prototypes: Construct an embodied set structure}

Algorithm 1: Pretrain agent-environment interaction models (embodied agent-state construction)
Given dataset with domain labels, how to construct the agent-environment interaction models .


Embodied agent-state set = generally reusable agent-environment interaction model
This set has several properties.
1, it's transferrable across domains defined by non-stationarity operators. 


\subsection{Re-use: a backbone for general downstream task learning}
There are three steps when reusing the pre-trained model in downstream task learning.

\paragraph{(1) Stability--Retain previous knowledge: Embodied Feature Projection}
asdfasdf

\paragraph{(2) Plasticity--Adapt to changes: Projected Bellman Updates}

\paragraph{(3) Put together--Downstream task learning: DQN-embodied version}

Algorithm 2: Reuse: DQN-embodied version as an example
Given a new downstream task, how to reuse... DQN example.


==> sections/performance_copy.tex <==
% \textbf{
% (1) Generally reusbale; (2) when reuse, learning downstream tasks based on the pre-trained model, it's important to have stability and plasticity. it's stable to non-stationarity during learning and after deployment due to feature projection that maintains the previous structure.  and adaptive to changes due to the Projected Bellman equation that approximates a new value function. 
% }

% \begin{figure}[bth]
%     \centering
%     	\begin{tabular}{@{}cc}
% 		{\includegraphics[height=1.3cm]{figs/fig3.pdf}}
% 		&{\includegraphics[height=1.3cm]{figs/fig6.pdf}}
% 	\end{tabular}
% 		\vspace{-5pt}
%     \caption{\footnotesize 3 curves as in one figure, curve remove title!. Row 1: compare ours to DQN, ER, 3RL. Row2: Compare ours to GPE/GPI, 1,2, VAE.\normalsize} %To ensure the evaluation environments are the consistent across different methods and multiple runs, we set a fixed random seed in each evaluation environment.}
%     \label{fig:learningcurve}
%     \vspace{-5pt}
% \end{figure}
 
\begin{figure*}[t]
 	\setlength{\belowcaptionskip}{-10pt}
	\centering
	\includegraphics[width=0.95\textwidth]{figs/fig2.pdf}
	\caption{\footnotesize \textbf{A:} Environments for collecting the pre-training dataset with different room layouts and random objects (keys, doors, coloured balls) for the agent to interact with. \textbf{B:} Downstream task ``goal-reaching'' uses the same environment as to pre-training but with a new task objective ``reach the green goal'' defined by the new reward function. \textbf{C:} Downstream task ``picking up the grey box'' uses a changed environment (locked door, grey box, coloured triangles are unseen during pre-training), and obviously a changed task objective. This task is challenging for vanilla RL agents when learning from scratch. \textbf{D:} Downstream task ``putting the green key near the yellow ball'' uses a changed environment (coloured triangles unseen during pre-training), changed task objective, and changed sensor modality by adding textual observations. Note this task requires text prompts otherwise it is difficult to solve by a vanilla RL agent\citep{minigrid} \normalsize}
 %     \vspace{-3.5mm}
	\label{fig:exp_setup}
\end{figure*} 

\subsection{Generality of re-use: a backbone for downstream task learning}
We conduct the \textit{generality test} by gradually adding differences between the downstream tasks and the pre-trained tasks. Fig. \ref{fig:exp_setup} gives an overview of task setup in the below three tests. 

\begin{figure}[]
    \centering
    	\begin{tabular}{@{}ccc}
     \footnotesize \textbf{A} change task objectives & \textbf{B} + change environments & \textbf{C} + change sensor modalities\\
		{\includegraphics[height=3.cm]{figs/test.pdf}}
		&{\includegraphics[height=3.cm]{figs/test.pdf}}
		&{\includegraphics[height=3.cm]{figs/test.pdf}}
	\end{tabular}
% 		\includegraphics[width=0.9\textwidth]{figs/updated/main_legend_update.pdf}
		\includegraphics[width=0.8\textwidth]{figs/test_legend.pdf}
		\vspace{-5pt}
    \caption{\footnotesize 3 curves as in one figure, curve remove title!. Row 1: compare ours to DQN, ER, 3RL. Row2: Compare ours to GPE/GPI, 1,2, VAE.\normalsize} %To ensure the evaluation environments are the consistent across different methods and multiple runs, we set a fixed random seed in each evaluation environment.}
    \label{fig:learningcurve}
    \vspace{-5pt}
\end{figure}

\textbf{Baselines:} We compare our methods to the following baselines. (1) Without pre-training: vanlilla DQN~\citep{Mnih2013PlayingAW}; (2) Reuse the pre-training dataset: experience replay (ER) which reuses the whole dataset $\mathcal{D}$ in the buffer to alleviate the forgetting issue~\citep{Rolnick2019ExperienceRF}; (3) Reuse a pre-training backbone: VAE~\citep{kingma2013auto}+DQN is used as a backbone for downstream task learning; (4) Reuse the pre-trained successor features (SF): GPE/GPI~\citep{barreto2020fast} method is used to learn the downstream task where during GPE, we use linear regression to estimate the new task weights based on our pre-trained cross-domain transferable SF $\phi^{\pi_{0}}(.;\theta_{sf})$.

We test the downstream task learning performance of all methods by evaluating the success rate every 10K steps using 100 independent runs with different random seeds.
% As shown in Fig. \ref{fig:eval_aim_generality}, we aim to examine \textbf{the generality} of our method by testing how well our proposed agent-environment interaction model as a general backbone, can boost downstream task learning in three heterogeneous task settings, as listed below. 

% \begin{wrapfigure}{r}{0.5\textwidth}
%     \centering
%     \includegraphics[width=0.5\textwidth]{figs/fig3.pdf}
%     \caption{\footnotesize Evaluation purpose of Sec. 5.1. \normalsize}
%     \label{fig:eval_aim_generality}
%     \vspace{-3.5mm}
% \end{wrapfigure}


\paragraph{(1) Task adaptation: changed task objective}
As shown in Fig. \ref{fig:exp_setup}B, the downstream task has the same environment as in pre-training. The task objective ``reach the green goal'' is defined by assigning a reward function: $r(x, a, x')=10$ if the goal is reached. Recall that this task objective is unseen during pre-training.  Results are shown in Fig. \ref{fig:learningcurve}\textbf{A} that our methods outperforms the 4 baselines. 
% Basic setting: changed task objectives.
% (1) No pre-training, just use the previous experience as they are:
%     - DQN: Learning from scratch
%     - ER: put offline dataset in the replay buffer, and use DQN
%     - 3RL: ER+RNN, put in replay buffer, + RNN structure.
%     - Plot their online learning performance, for every 10K samples used during training.
% (2) Has pretraining
%     - GPE (Regression-non-linear)/GPI
%         - Pretraining: SF
%         - Reuse: (1) train w regressor (use our learned SF and the repgress W); (2) GPI
%         - Plot: GPI resuls (use return) (minigrid reward must have penalty at each step), for every 10K samples used in the w regression.
%         - How to collect data: Uniform policy.
%         - To avoid any linearity assumptions, we use a 3-layer MLP with Relu activations to regress the W.
%         - Can generalize, since considering a reward function space spanned by SF feature, 
%     - GPE (TD-non-linear) / GPI
%         - GPE: do not use our pretrained SF, pre-train 20 policies on 20 resulting MDPs, calc value function for the 20 policies.
%         - Reuse: (1) learn value function by TD learning; (2) GPI
%         - Plot: GPI resuls (use return) (minigrid reward must have penalty at each step), for every 10K samples used in the w regression.
%         - Can not generalize well, since do not consider a reward function space spanned by SF features
%     - VAE + DQN
%         - Plot DQN performance, for every 10K samples used.
% Baselines: No need to use two figs to differentiate them.
% - learn from scratch
% - use the pre-collected dataset: DQN, ER, 3RL
% - use pre-training: VAE+DQN, GPE (Regression-non-linear)/GPI, GPE (TD-non-linear)/GPI

% Results to show:
% Return - sample efficiency curves: of our method, and 6 baselines.

\paragraph{(2) General task adaptation: changed task objective + changed environment}
We keep testing the generality of our proposed method by changing both the environment and the task objective. The environment is changed by adding a door to the bottleneck hallway and different colored triangles where the agent has never seen before. The task objective is now changed to ``pick up the grey box'' that the agent needs to firstly pick up the key, unlock the door and then pick up the grey box. The reward function is defined as $r(x, a, x')=$ 1 (if pick up the key or unlock the door), 10 (if succeed).



    - Unlock pickup task, need to unlock the door (by picking up the key), and pick up a box.
    - It only has two rooms!
    - This task can be solved without relying on language.

Results to show:
Success rate - sample efficiency curves: of our method, and 6 baselines.

\paragraph{(3) More general task adaptation: changed task objective + changed environment + changed sensor modalities}
Baselines: 
- No pretraining: DQN, ER, 3RL, 
- With pretraining: GPE-linear/GPI, GPE-non-linear/GPI, VAE+DQN
    - GPE, GPI will perform very bad, since env dynamic changed.

How: find a task is difficult to solve without text for vanlila RL methods.
MiniGrid-LockedRoom-v0
- The agent needs to understand the text, which tells it which room to get the key and go to which room to open the door. And then pick up a box.
- It has six rooms!
- This task is difficult since the agent needs to understand the textual mission info.

Results to show:
Success rate - sample efficiency curves: of our method, and 6 baselines.




\paragraph{(4) Deployment Robustness: robustness to non-stationarity during testing}
We wonder, how the trained policy based on our proposed model, is robust to non-stationarity during testing. To test, we manually change the environment slightly to add such non-stationarity.
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    	\begin{tabular}{@{}ccc}
		{\includegraphics[height=4cm]{figs/test2.png}}
	\end{tabular}
		\includegraphics[width=0.5\textwidth]{figs/test_legend.pdf}
		\vspace{-5pt}
    \caption{\footnotesize deployment stability to env changes. 100 Runs, each run random seed, then Slightly change the key to the left 1 cell to the current key position config. Test 6 baselines, and ours\normalsize} 
    \label{fig:213}
    \vspace{-5pt}
\end{wrapfigure}
No need any images to show the change.
Now, at B1, we train the unlock Pick Up one. We can directly use the ones trained in 5.1 (2).

We test the performance if we slightly change the key location, 10 random changes.
Baselines:
- No pretraining: DQN, ER, 3RL, 
- With pretraining: GPE-linear/GPI, GPE-non-linear/GPI, VAE+DQN
- GPE, GPI will perform very bad, since env dynamic changed.

Ours are more robust to non-stationarity after deployment of the policy.

Results to show:
Success rate during testing - sample efficiency curves: of our method, and 6 baselines.
Use a Table to show the result, NOT %直方图 以节省page 空间
sucess rate: 79+- 5 \% 
% \begin{wraptable}{r}{5.5cm}
% \caption{A wrapped table going nicely inside the text.}\label{wrap-tab:1}
% \begin{tabular}{ccc}\\\toprule  
% Method & Header-1 & Header-1 \\\midrule
% Success rate &3 & 5\\  \midrule
% 2 &3 & 5\\  \midrule
% 2 &3 & 5\\  \bottomrule
% \end{tabular}
% \end{wraptable} 

\subsection{Learning stability and plasticity: a backbone that handles non-stationarity}
As shown in Fig. \ref{fig:eval_stability_plasticity}, we aim to examine the learning \textit{stability-plasticity} analysis by a deep look at how well our proposed agent-environment interaction model, as a backbone for downstream task learning, can handle non-stationarity during training, testing, and in a continual learning setting. Specifically, we evaluation from the following perspectives.

\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/fig6.pdf}
    \caption{\footnotesize Evaluation purpose of Sec. 5.2. \normalsize}
    \label{fig:eval_stability_plasticity}
    \vspace{-3.5mm}
\end{wrapfigure}

Learned from past experience, will it make the resulting policy be more stable than learning from raw observations, or using other pre-traning methods, like VAEs?
How to do?
After the downstream task learning, choose the one learned from VAE, and the one learned using our method, and the one learned from scratch.
Now, let's change a part of the environment, see the performance. VAE, scratch, its success rate drops quickly, but ours stay robust.


\paragraph{(1) Learning stability: changing environment during downstream task training}
Now, let's continue our test. During reuse, when we train the downstream task, we will change the environment.
Baselines:
% - DQN: without env change. %这个不需要
- DQN: vanilla baseline.
- VAE + DQN: use the pre-trained VAE structure.
% - VAE + DQN without env change %这个不需要
\begin{wrapfigure}{r}{0.5\textwidth}
    \centering
    \includegraphics[width=0.5\textwidth]{figs/fig5.pdf}
    \caption{\footnotesize Fig. Left env at start --> train and get an optimal policy., Middle env changed at 30K completion, Right env changed at 60K. Say clearly, this is changed during training.\normalsize}
    %\label{fig:decentcem-a-architecture}
    %\vspace{-3.5mm}
\end{wrapfigure}

First, run DQN to see how many samples are required. During training, at 30\% of DQN samples (interaction steps), change the env once. at 70\% of DQN samples, change the env the second time. There are two changes during training.


Unlock Pick up, we change the key position at B2, B3, so it will change the environment.

Results to show:
Success rate - sample efficiency curves: of our method, and 6 baselines.


\paragraph{(2) Vanilla plasticity: continual learning in changing environments}
Let's continully update the policy.
Vanilla plasticity, we do not add anything special, just keep training the learned policy, by projecting to our embodied agent-state set. We show that, this vanlila version of DQN shows plasticity, that it quickly adapts to the new environment setting.

While the baseline, we compare, is learning from the raw state. it drops quickly.

Another baseline is EWC, it performs pretty well.

The last baseline is ours + EWC, it performs even better.

In the unlock and pick up task, just reuse the pretrained one in 5.1 (2).

Now we change the env (change the key position). We keep updating the policy trained in 5.1 (2). And we change the key position again, keep updating based on previous one.
Two changes.

Policy 1: the one trained from 5.1 (2)
Policy 2: change the env, and train based on policy 1.
Policy 3: change the env, and train based on policy 2.

Stability: there is no sudden drop of performance.
Plasticity: it can reach to high performance than the other ones. to achive good performance in the changed envs.

Baselines:
- DQN
- Ours (DQN-embodied)
- DQN + EWC
- Ours (DQN-embodied) + EWC

Ours, even without EWC, can show simliar performance to DQN + EWC.
Ours + EWC shows the best performance, that recovers quickly!!!!

Results to show:
Success rate during training - sample efficiency curves: of our method, and 6 baselines.
Needs to see a drop of performance. So need to show the curve.



\begin{figure}[bth]
    \centering
 \begin{tabularx}{1\textwidth}{>{\centering\arraybackslash}m{2.2cm} >{\centering\arraybackslash}m{4cm} >{\centering\arraybackslash}m{5.8cm}}
% \hline
\footnotesize
~ & A Learning stability & B Vanilla plasticity\\
% \hline
\footnotesize Compared to vanilla learning methods & {\includegraphics[height=3cm]{figs/test.pdf}} &  {\includegraphics[height=3cm]{figs/test.pdf}} \\
% \hline
\footnotesize Compared to EWC learning methods & {\includegraphics[height=3cm]{figs/test.pdf}} & {\includegraphics[height=3cm]{figs/test.pdf}} \\
% \hline
\end{tabularx} \normalfont
% 		\includegraphics[width=0.9\textwidth]{figs/updated/main_legend_update.pdf}
		\includegraphics[width=0.8\textwidth]{figs/test_legend.pdf}
		\vspace{-5pt}
    \caption{\footnotesize 2 curves as in one figure, curve remove title!. \normalsize} %To ensure the evaluation environments are the consistent across different methods and multiple runs, we set a fixed random seed in each evaluation environment.}
    \label{fig:learningcurve}
    \vspace{-5pt}
\end{figure}

% \paragraph{(3) Why it supports learning stability and plasticity}
% Why is that?

% Though we change the enironmnet, but we built based on the long term predictions representations, so that the projected representation does not change too much.

% For example, this is the environment, 
% VAE, raw state features, ...
% VAE, will have a big drift since it overfits to previous dataset distributions. because of the change, it forgets about previously learned bottleneck, passways.
% Raw state --> embedding, just changes dramatically.

% By projecting on this abstraction structure, it gains plasticity, also maintains stability.

% Since it is built based on the agent's own experience.

% Ours, maintain stable

% % Color map of the four rooms, ours, continue have high value on pass ways, and ignore the changes. This shows 
% % We don't update the backbone, can it show plasticity?
% % in the future, we will update the backbone.
% plot the value function's output based on ours model, VAE model, and just raw observations.
% Plot (1): changed the environment, the initial value function's output of ours (DQN-embodied). the initial value function is good for the previous environment.
%         - DQN, VAE based ones, the value function's output makes wrong predictions on unchanged cells
%         - Ours, makes correct predictions on unchanged cells.
%      (2): after a few steps 10K training, newly trained value function
%         - DQN, VAE beased ones, the value function's output still are confused, not adapt to the changed cell, i.e., the new key location.
%         - Ours, makes almost increased, and correct predictions on the changed cell.
%      (3): plot the newly trained value function's output - initial value function's output
%         - DQN, VAE based ones, unchanged cells still show changes like noise, no any patterns. Changed cells still show this.
%         - Ours, unchanged ones, almost zero value prediction changes. Changed ones, show positive, and negative changes.
% (3) show clearer how downstream task learning agent (DQN) based on our model, can have vanilla stability-plasticity.

% How many experiments/trainings do I need? Make a table and chart.

 
%  Q value computed by: max Q (of all the 6 acctions), norm(|Q(s,a1), Q(s, a2), Q(s, a3), ...|)-infinity.
%  \begin{figure*}[tpb]
%     \centering
%     \includegraphics[width=0.99\textwidth]{figs/fig7.pdf}
%     \caption{\footnotesize as shown above, another evidence that it supports stability and plasticity. It supports stability by feature projection, that retrain previous learned structure (As shown in Fig. 8, that it maintains the agent-state structure from Train A to Train B, by always doing feature projection on the embodied state.), as a reuslt, even env changes from A to B, at the begining of train B, it maintains good value predictions, and this is maintained until the end of train B. It supports plasticity by Projected Bellman Updates that it adapts to the new changes (as shown in Fig 7, that it adapts to the changes of the key positions. It's initially wrong at the changed key positions, and wrong at the preivous key positions. But at the end of train B, it adapts to the new good values. \normalsize}
%     %\label{fig:decentcem-a-architecture}
%     %\vspace{-3.5mm}
% \end{figure*}


\subsection{Summary of results}


